A Sentence Compression Based Framework to Query-Focused Multi-Document Summarization

We consider the problem of using sentence compression techniques to facilitate query-focused multi-document summarization. We present a sentence-compression-based framework for the task, and design a series of learning-based compression models built on parse trees. An innovative beam search decoder is proposed to efficiently find highly probable compressions. Under this framework, we show how to integrate various indicative metrics such as linguistic motivation and query relevance into the compression process by deriving a novel formulation of a compression scoring function. Our best model achieves statistically significant improvement over the state-of-the-art systems on several metrics (e.g. 8.0% and 5.4% improvements in ROUGE-2 respectively) for the DUC 2006 and 2007 summarization task.

==> parsetree.tex <==
\begin{figure}
\hspace{2mm}
\includegraphics[width=70mm,height=45mm]{trimParseTree.png}
\vspace{-5mm}
\caption{\footnotesize Diagram of tree-based sentence compression. The node and the subtrees it subsumes to be dropped are grayed out. In this exmaple, the node of the entire gray part with a tag of ``PP" is labeled as \textsc{Remove}. All of its siblings are labeled as \textsc{Retain}, and its parent is tagged as \textsc{Partial}. The linearization of this trimmed parsing tree is realized as ``Malaria causes millions of deaths."}
\label{fig:parsetree}
\vspace{-3mm}
\end{figure}

\begin{figure}
\hspace{-2mm}
\includegraphics[width=85mm,height=40mm]{beamSearchTree.png}
\vspace{-10mm}
\caption{\footnotesize Example of beam search decoder. In a postorder traversal, the three nodes with hypotheses in box are visted in a bottom-up order. The hypotheses are ranked according to the scores in the parentheses. Beams for other nodes are omitted. }
\label{fig:beamsearch}
\vspace{-3mm}
\end{figure}


